DMSA -- Dense Multi Scan Adjustment for LiDAR Inertial Odometry and Global Optimization

We propose a new method for fine registering multiple point clouds simultaneously. The approach is characterized by being dense, therefore point clouds are not reduced to pre-selected features in advance. Furthermore, the approach is robust against small overlaps and dynamic objects, since no direct correspondences are assumed between point clouds. Instead, all points are merged into a global point cloud, whose scattering is then iteratively reduced. This is achieved by dividing the global point cloud into uniform grid cells whose contents are subsequently modeled by normal distributions. We show that the proposed approach can be used in a sliding window continuous trajectory optimization combined with IMU measurements to obtain a highly accurate and robust LiDAR inertial odometry estimation. Furthermore, we show that the proposed approach is also suitable for large scale keyframe optimization to increase accuracy. We provide the source code and some experimental data on https://github.com/davidskdds/DMSA_LiDAR_SLAM.git.

==> backup.tex <==
\begin{figure*}[htbp]
\begin{subfigure}{0.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=0.71\linewidth,trim=0 0 0 50,clip]{figures/basement_bird.pdf}  
  \caption{ }
  \label{fig:process1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{figures/cloister_bv.pdf}  
  \caption{ }
  \label{fig:process2}
\end{subfigure}\newline

\begin{subfigure}{0.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.81\linewidth]{figures/parkland_mound.pdf}  
  \caption{ }
  \label{fig:process1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.73\linewidth,angle=-2.5,origin=c]{figures/stairs.pdf}  
  \caption{ }
  \label{fig:process2}
\end{subfigure}
\caption{Resulting keyframe point clouds.}
\label{fig:process}
\end{figure*}
